Scalable Variational Gaussian Processes via Harmonic Kernel Decomposition

We introduce a new scalable variational Gaussian process approximation which provides a high fidelity approximation while retaining general applicability. We propose the harmonic kernel decomposition (HKD), which uses Fourier series to decompose a kernel as a sum of orthogonal kernels. Our variational approximation exploits this orthogonality to enable a large number of inducing points at a low computational cost. We demonstrate that, on a range of regression and classification problems, our approach can exploit input space symmetries such as translations and reflections, and it significantly outperforms standard variational methods in scalability and accuracy. Notably, our approach achieves state-of-the-art results on CIFAR-10 among pure GP models.

==> kern-tex/background-legacy.tex <==
\section{Background}

Throughout the paper, we use lowercase characters $a$ to represent scalars, bold lowercase characters $\ba$ to represent vectors, and bold uppercase characters $\bA$ and to represent matrices. We use $\bA^{\top}$ to represent transposes, and use $\bA^H$ to represent the conjugate transposes.

\subsection{Fourier Transform and Fourier Series}
Fourier analysis \citep{baron1878analytical} is concerned in representing the functions as sums of harmonic series. For an integrable function $f$ with domain $\Reals^d$, its Fourier transform returns a function $\hat{f}$ of the frequence $\bomega$,
\begin{align}
    \hat{f}(\bomega) = \int_{\mathbb{R}^d} \exp(-2\pi i \bomega^\top\bx) f(\bx) \mathrm{d}\bx,
\end{align}
where $\hat{f}(\bomega) \in \Complex$, whose magnitude characterizes the amount of the frequency $\bomega$ present in $f$. The inverse Fourier transform maps $\hat{f}$ back to $f$, $f(\bx)  = \int_{\mathbb{R}^d} \exp(2\pi i \bomega^\top\bx) \hat{f}(\bomega) \mathrm{d}\bomega$.

Fourier analysis can be performed over finite sequences as well, via the discrete Fourier transform (DFT). Specifically, given a finite sequence $\bx = [\bx_0, ..., \bx_{N-1}]^{\top}$, DFT computes the Fourier series $\hat{\bx} = [\hat{\bx}_0, ..., \hat{\bx}_{N-1}]^{\top}$, 
\begin{align}
   \hat{\bx}_{m} = \frac{1}{N}\sum_{n=0}^{N-1} \bx_n e^{-i\frac{2\pi n m}{N}}, \; m=0,...,N-1, 
\end{align}
Let $\bF = [\frac{1}{N} e^{-i\frac{2\pi n m}{N} } ]_{n,m=0}^{N-1} \in \Complex^{N \times N}$, DFT can be written compactly as : $\hat{\bx} = \bF \bx$. We can also compute the inverse discrete Fourier transform: $\bx = \bF^{-1}\hat{\bx}$, where $\bF^{-1} = [e^{i\frac{2\pi nm}{N}}]_{n,m=0}^{N-1}$. More generally, if $\bX \in \Complex^{N_1 \times \cdots \times N_k}$ is a tensor, DFT computes $\hat{\bX} \in \Complex^{N_1 \times \cdots \times N_k}$,
\begin{align}
    \hat{\bX}[m_1, ..., m_k] = \frac{1}{N} \sum_{n_1, ..., n_k} X[n_1, ..., n_k] \prod_{j=1}^k e^{-i\frac{2\pi n_j m_j}{N_j}}, \notag 
\end{align}
where $N = \prod_{j}N_j$ and $\hat{\bX}$ is the frequency tensor of the same shape as $\bX$.

\subsection{Gaussian Processes}
Given the input domain $\xdomain$ and a kernel function $k: \xdomain \times \xdomain \to \Reals$, a zero-mean Gaussian process \citep{rasmussen2006gaussian} $\GP(0, k)$ is a distribution $p(f)$ over functions $\xdomain \to \Reals$. For any finite set $\{\bx_1, ..., \bx_n\} \subset \xdomain$, the function values $\bbf = (f(\bx_1), f(\bx_2), ..., f(\bx_n))$ have a multivariate Gaussian distribution. %Gaussian processes are parameterized by a covariance function or kernel function $k(\cdot, \cdot)$. The marginal distribution of function values is given by
\begin{equation}
\bbf \sim \mathcal{N}(\bzero, \mathbf{K}_{\bbf \bbf}), \notag 
\end{equation}
where $\mathbf{K}_{\bbf \bbf} = [k(\bx_i,\bx_j)]_{i,j=1}^n$. The observation $y$ is generated by the likelihood $p(y|f)$. For regression problems, the likelihood usually models independent Gaussian noise: $y = f(\bx) + \epsilon, \quad \epsilon \sim \mathcal{N}(0, \sigma^2)$. Let  $(\bX, \by)$ be the training set of size $N$, the posterior $p(\bbf^{\star}|\by)$ is an explicit Gaussian under Gaussian likelihoods,
\begin{align}
\normal( \bK_{\star \bbf}(\bK_{\bbf \bbf} + \sigma^2\bI_N)^{-1}\by, \bK_{\star \star} - \bK_{\star \bbf}(\bK_{\bbf \bbf} + \sigma^2\bI_N)^{-1}  \bK_{\bbf \star}), \notag
\end{align}
%$\tilde{\bK}_{\bbf \bbf} = \bK_{\bbf \bbf} + \sigma^2\bI_N$, the posterior is an explicit Gaussian under Gaussian likelihoods,
%\begin{align}
%\bbf^{\star}|\by \sim \normal( \bK_{\star \bbf}\tilde{\bK}_{\bbf \bbf}^{-1}\by, \bK_{\star \star} - \bK_{\star \bbf}\tilde{\bK}_{\bbf \bbf}^{-1}  \bK_{\bbf \star}), \notag
%\end{align}
where $\bbf^{\star}=f(\bX^{\star})$ are function values at test locations. However, the posterior involves inverting the kernel matrix, which requires $\bigO(N^3)$ computational costs.

Sparse variational Gaussian Processes (SVGP) \citep{titsias2009variational, hensman2013gaussian} use inducing point for scalable GP inference. Let $\bZ = [\bz_1, ..., \bz_M]^{\top} \in \Reals^{M \times d}$ be $M$ inducing locations, and $\bu = f(\bZ)$. SVGP considers an augmented joint likelihood, $p(f, \bu) = p(f | \bu) p(\bu)$, and a variational posterior $q(f, \bu) = p(f | \bu) q(\bu), q(\bu)=\normal(\bmu, \bS)$. The variational posterior is optimized by maximizing the Evidence Lower Bound (ELBO):
\begin{align}
    \elbo \defas \expect_{q(f, \bu)} [\log p(\by|f, \bX)] - \KL{q(\bu)}{p(\bu)}.
\end{align}
Since $\log p(\by|f, \bX) = \sum_{i=1}^N \log p(\by_i|f, \bx_i)$, the ELBO admits stochastic optimizations. Therefore, the SVGP reduces the computational costs from $\bigO(N^3)$ to $\bigO(M^3)$.

%
%\subsection{Kernel Fourier Analysis}
%
%\textbf{Bochner's Theorem} \citep{bochner1959lectures} establishes a bijection between complex-valued stationary kernels $k(\bx, \bx')=\tau(\bx-\bx')$ and positive finite measures using Fourier transform, thus providing an approach to analyze stationary kernels in the spectral domain \citep{wilson2013gaussian, kom2015generalized, remes2017non, samo2015generalized}.
%
%\begin{theorem}[Bochner's]\label{thm:bochners}
%A complex-valued function $k$ on $\mathbb{R}^d$ is the covariance function of a weakly stationary mean square continuous complex-valued random process on $\mathbb{R}^d$ if and only if it can be represented as 
%\begin{equation}
%    k(\bx, \bx') = \int_{\mathbb{R}^d} \exp(2\pi i \bomega^\top(\bx - \bx')) S(\bomega) \mathrm{d}\bomega
%\end{equation}
%where $S$ is called the spectral density or power spectrum of $k$. $S$ and $k$ are Fourier duals.
%\end{theorem}
%
%\textbf{Spherical Harmonics} \citep{thomson1888treatise, morimoto1998analytic} provides the spectral decomposition for zonal kernels $k(\bx, \bx') = \tau(\bx^{\top}\bx')$ on the hypersphere $\Sphere^{d-1}$, as a counterpart of the stationary kernels on $\Reals^d$.
%
%\begin{theorem} Any zonal kernel $k$ one the sphere $\Sphere^{d-1}$ can be decomposed as,
%\begin{align}
%    k(\bx, \bx') = \sum_{l=0}^{\infty}\sum_{m=1}^{N^d_l} \hat{a}_{l,m} Y_{l,m}(\bx)Y_{l,m}(\bx'),
%\end{align}
%where $\bx, \bx' \in \Sphere^{d-1}$ and $\hat{a}_{l,m}$ are positive coefficients. $Y_{l,m}$ denote the spherical harmonics and $N^d_l$ is the number of spherical harmonics for degree $l$.\end{theorem}
%For example when $d=2$, $\bx \in \Sphere^{1}$ can be represented by its angle $\theta$, then $Y_{l,m}(\bx) \in \mathrm{span}\{\cos l \theta, \sin l\theta \}$. Thus the spherical harmonics form a \emph{Fourier decomposition on the sphere}. Because the spherical harmonics are mutually orthogonal with respect to the RKHS norm, $\innerprod{Y_{l,m}(\bx)}{Y_{l',m'}(\bx)}_{\rkhs_k} \propto \delta_{ll'} \delta_{mm'}$, it is adopted as the variational features for scalable Gaussian process \citep{dutordoir2020sparse}. 

==> kern-tex/kernel-legacy.tex <==

\section{Orthogonal Kernel Decomposition}\label{sec:kern-decomp}
In this section we establish the framework to conduct kernel Fourier analysis, and prove that the kernel Fourier series leads to the orthogonal kernel decomposition.

\textbf{$T$-Periodic Transformation $G$.} A function $G: \xdomain \to \xdomain$ is $T$-periodic if $T$ is the smallest integer such that,
\begin{align}
    \forall \bx \in \xdomain, G^T (\bx) \defas \overbrace{G \circ \cdots \circ G}^{T} (\bx) = \bx,
\end{align}
So $T$ consecutive applications of $G$ is the identity operator. Throughout this paper, we use $G^t$ to represent $t$ consecutive applications of $G$ for $t \in \Nats$.

\textbf{$G$-Invariant kernels.} A kernel function $k: \xdomain \times \xdomain \to \Complex$ is $G$-invariant if,
\begin{align}
    \forall \bx, \bx' \in \xdomain, k(G(\bx), G(\bx')) = k(\bx, \bx'),
\end{align}
For example, a polynomial kernel $k(\bx, \bx')=(\bx^{\top}\bx'+c)^t$ is invariant to the rotation transformations.

\textbf{Kernel Fourier Series.} We define $T$ functions $k_t: \xdomain \times \xdomain \to \Complex, t=0,...,T-1$, using the Fourier series of the sequence $[k(\bx, G^0(\bx')), ..., k(\bx, G^{T-1}(\bx'))]$. Specifically, the $t$-th function represents the $t$-th frequency harmonics from DFT,
\begin{align}
    k_t(\bx, \bx') =  \sum_{s=0}^{T-1} \bF_{t, s} k(\bx, G^s(\bx')),
\end{align}
where $\bF = [\frac{1}{T} e^{-i\frac{2\pi t s}{T} } ]_{t,s=0}^{T-1}$ is the DFT matrix.

\subsection{Orthogonal Kernel Decomposition}
In this subsection we present our main result, that the kernel Fourier series form an orthogonal kernel sum decomposition of the kernel $k$.

\begin{theorem}[Kernel Sum Decomposition.] 
\begin{align}
    k(\bx, \bx') = \sum_{t=0}^{T-1} k_t(\bx, \bx').
\end{align}
Moreover, for $t=0,...,T-1$, $k_t$ is a Hermitian kernel.
\end{theorem}

\begin{proof}
The equality can be directly proven,  
\begin{align}
   \sum_{t=0}^{T-1} k_t(\bx, \bx')
    &= \sum_{t=0}^{T-1} \sum_{s=0}^{T-1} \frac{1}{T}e^{-i\frac{2\pi st}{T}} k(\bx, G^s(\bx')) \notag \\
    &=\frac{1}{T}  \sum_{s=0}^{T-1} k(\bx, G^s(\bx')) \sum_{t=0}^{T-1} e^{-i\frac{2\pi st}{T} } \notag \\
    &= \frac{1}{T}  \sum_{s=0}^{T-1} k(\bx, G^s(\bx')) T\delta_{s} = k(\bx, \bx'). \notag
\end{align}
To prove that $k_t$ is a kernel, we claim that $k_t(\bx, \bx') = \bF_{t,:}^H \bK \bF_{t,:}$, where $\bK = [k(G^{s_1}(\bx), G^{s_2}(\bx'))]_{s_1, s_2=0}^{T-1}$. Expanding the matrix vector products,
\begin{align}
    &\frac{1}{T^2}\sum_{s_1=0}^{T-1}\sum_{s_2=0}^{T-1} e^{-i\frac{2\pi t}{T}(s_2-s_1) }k(G^{s_1}(\bx), G^{s_1 + (s_2-s_1)}(\bx')) \notag \\
    &=\frac{1}{T}\sum_{s_0=0}^{T-1} e^{-i\frac{2\pi t }{T}s_0 }k(\bx, G^{s_0}(\bx')) = k_t(\bx, \bx'), \notag 
\end{align}
where we changed the variable $s_2-s_1$ to $s_0$. Furthermore, since $k$ is a kernel and $\bK$ is positive semidefinite,  we conclude that $k_t(\bx, \bx') = \bF_{t,:}^H \bK \bF_{t,:}$ is a kernel as well.
\end{proof}

Besides the kernel sum decomposition, we further show that the kernels $k_t, t=0,...,T-1$ are orthogonal to each other, as identified by the following lemma.

\begin{lemma}[Orthogonality]\label{lem:ortho} For any $0\leq t_1 \neq t_2 \leq T-1$, let $\rkhs_k, \rkhs_1, \rkhs_2$ be the RKHSs corresponding to the kernel $k, k_{t_1}, k_{t_2}$, respectively. Then for any  $f \in \rkhs_{1}$ and $g \in \rkhs_{2}$, $\innerprod{f}{g}_{\rkhs_k} = 0$.
\end{lemma}
The proof of this lemma can be found in Subsection~\ref{app:proof:ortho} in the appendix. Because the $\rkhs_k$ inner product of $f \in \rkhs_{1}, g \in \rkhs_{2}$ is always zero, we immediately obtain that the RKHSs for $k_t$ are disjoint expect the function $f \equiv 0$.
\begin{proposition}[Disjoint] For $t=0,...,T-1$, let $\rkhs_t$ be the RKHS associated with $k_t$, then for any $0\leq t_1 \neq t_2 \leq T-1$,
\begin{align}
    \rkhs_{t_1} \cap \rkhs_{t_2} = \{0\},
\end{align}
\end{proposition}

The kernel summation and the orthogonality of RKHSs, translate to the RKHS orthogonal sum decomposition as follows,
\begin{theorem}[RKHS Orthogonal Sum Decomposition.] The RKHS $\rkhs_k$ admits an orthogonal sum decomposition,
\begin{align}
    \rkhs_k = \bigoplus_{t=0}^{T-1} \rkhs_{k_t},
\end{align}
Specifically, for any function $f \in \rkhs_k $, $f$ has the unique decomposition $f = \sum_{t=0}^{T-1} f_t, f_t \in \rkhs_{k_t}$,
\begin{align}
    f_t(\bx) = \int k_t(\bx, \by) f(\by) d\bx,
\end{align}
The RKHS norm of $f$ equals to,
\begin{align}
    \|f\|^2_{\rkhs_k} = \sum_{t=0}^{T-1} \|f_t\|^2_{\rkhs_{k_t}}. 
\end{align}
\end{theorem}

\subsection{Examples of Kernel Fourier Series}\label{subsec:example}
\textbf{A Teaser Example.} We start with a toy problem for illustrating the kernel decomposition. We use $\theta \in [0, 2\pi)$ as the input, then $G(\theta) = (\theta + \frac{2\pi}{T}) \mod 2\pi$ is  $T$-periodic.
the kernel $k(\theta, \theta') = e^{-i(\theta - \theta')} + e^{-2i(\theta - \theta')}$ is then $G$-invariant. The kernel Fourier series can be explicitly obtained as, $k_{1}(\theta, \theta') = e^{-i(\theta - \theta')}$, $k_{2}(\theta, \theta') = e^{-2i(\theta - \theta')}$, and $k_t = 0$ otherwise. The RKHSs of $k_1$ and $k_2$ contain periodic functions of period $2\pi$ and $\pi$, respectively. Therefore, the kernel Fourier series decompose the original RKHS $\rkhs_k$ into orthogonal RKHSs based on the frequencies.

\textbf{Inner-product kernels} are kernels of the form,
\begin{align}
    k(\bx, \bx') = \kappa(\bx^H\bx, \bx^H\bx', \bx'^H\bx'),
\end{align}
where the function $\kappa$ assures $k$ being positive semi-definite. For any matrix $\bR \in \Complex^{d \times d}$, which is unitary $\bR \bR^{*} = \bI$ and $\bR^{T} = \bI$, the mapping $G(\bx) = \bR \bx$ is a $T$-periodic transformation. Because $\bR$ is unitary, the kernel $k$ is $G$-invariant,
\begin{align}
    k(G(\bx), G(\bx')) &= \kappa(\bx^H \bR^H \bR \bx, \bx^H \bR^H \bR \bx', \bx'^H \bR^H \bR  \bx') \notag \\
    &= \kappa(\bx^H\bx, \bx^H\bx', \bx'^H\bx') \notag,
\end{align}
Therefore, we can compute the kernel Fourier series $k_t$. $k_t$ captures the $t$-th harmonic of the kernel $k$ along the trajectory of rotations $\bR$.

\textbf{Stationary kernels} are kernels of the form,
\begin{align}
    k(\bx, \bx') = \kappa(\bx - \bx'),
\end{align}
where $\kappa$ is a positive-type function. Let $T=2$ and $G(\bx) = -\bx$, then $G$ is $T$-periodic. For real kernels whose $k(\bx, \bx') \in \Reals$, the kernel is symmetric $k(\bx, \bx')=k(\bx', \bx)$. Then $k$ is $G$-invariant,
\begin{align}
    k(G(\bx), G(\bx')) = \kappa(\bx' - \bx) = k(\bx', \bx) = k(\bx, \bx'). \notag 
\end{align} 
Notably, the inner-product kernels are invariant to negations as well, thus $G(\bx)=-\bx$ is applicable to both stationary kernels and inner-product kernels.

%\textbf{Periodic kernels} models periodic functions,
%\begin{align}
%    k(\bx, \bx') = \sigma^2 \exp(-\frac{\sin^2(\pi \|\bx-\bx'\|_2 / \gamma)}{2l^2}),
%\end{align}
%where $\gamma$ is the period parameter. Let $G(\bx) = \bx + \frac{\gamma}{T}$

%
%\subsection{Stationary Kernel Decomposition}
%Stationary kernels are kernels of the form,
%\begin{align}
%    k(\bx, \bx') = \tau(\bx - \bx'),
%\end{align}
%We assume $\tau$ is continuous. We assume the original input space $\xdomain = [0, a]^d$, and we define an extended input space $\tilde{\xdomain} = [0, 2a]^d$. The kernel $\tilde{k}$ on $\tilde{\xdomain}$ is an extension of the kernel $k$. Specifically, $\tilde{k}(\bx, \bx') = \tau(\gamma(\bx - \bx'))$, where $\gamma$ is an elementwise function as shown in the following,
%\begin{align}
%    \gamma(x) = \begin{cases}
% -(x + 2a) & -2a \leq x < -a \\
% x & -a \leq x \leq a \\
% 2a-x & a < x \leq 2a
% \end{cases}
%\end{align}
%%
%%\begin{figure}[h]
%%\centering
%%\includegraphics[width=0.5\textwidth]{figures/gamma.pdf}
%%\caption{The gamma Function.}
%%\end{figure}
%Because the gamma function is identity within $[-a, a]$, $\tilde{k}(\bx_1, \bx_2) = k(\bx_1, \bx_2)$ when $\bx_1, \bx_2 \in \xdomain$.
%\begin{lemma}\label{lem:tilde-k}$\tilde{k}$ is a kernel.
%\end{lemma}
%
%
%%We also present a useful property of $k$, if $\bx' \geq 0$, $\tilde{k}(\bx, \bx'-2a) = \tilde{k}(\bx, \bx')$. To prove it, notice
%%\begin{align}
%%    \gamma(x - x' + 2a) =  -\gamma(x - x') = \gamma(x' - x),
%%\end{align}
%%Thus $\tilde{k}(\bx, \bx'-2a) = \tilde{k}(\bx', \bx) = \tilde{k}(\bx, \bx')$. Similarly, if $\bx' < 0$, then $\tilde{k}(\bx, \bx'+2a) = \tilde{k}(\bx, \bx')$.
%%\ssy{Not very happy about this, if $k$ maps to $\Complex$, then it is wrong.}
%
%Given an integer $T$, we define the mapping,
%\begin{align}
%    G(x) = x + \frac{2a}{T}  - 2a \times \mathbb{I}[\bx + \frac{2a}{T} > 2a],
%\end{align}
%Because the domain $[0, 2a]$ is of length $2a$, $G^T(\bx) = \bx$, i.e., $G$ is a $T$-periodic transformation. Furthermore, we can show that the kernel $\tilde{k}$ is $G$-invariant as well:
%\begin{lemma}[Stationary $G$-invariance]\label{lem:stationary-g-invariance} The kernel $\tilde{k}$ is $G$-invariant.
%\end{lemma}
%Please refer to Subsection~\ref{app:proof:k-kern} and Subsection~\ref{app:proof:sta-g-inv} in the appendix for the proofs of the preceding lemmas.

\subsection{Multi-dimensional Transformations}\label{subsec:multi-dim}
In the previous subsections we considered the Fourier series along one transformation trajectory: $k(\bx, G^0(\bx')), k(\bx, G^1(\bx')), ..., k(\bx, G^{T-1}(\bx'))$. Furthermore, we can extend the single transformation sequence to a multidimensional transformation tensor map, which would provide a tensor sum decomposition of the kernel. Specifically, let $T_1, ..., T_M \in \Nats$ and $G_m$ is a $T_m$-periodic transformation for $m=1,...,M$, respectively. We further assume that all transformations commute, i.e., $\forall 1\leq m_1, m_2 \leq M$, 
\begin{align}
\forall \bx \in \xdomain, G_{m_1} (G_{m_2} (\bx)) =  G_{m_2} (G_{m_1} (\bx)) ,
\end{align}
Due to the commuting property, we can use indices $(t_1, ..., t_M)$ and the character $G$ to represent applying each $G_m$ by $t_m$ times, 
\begin{align}
    G^{(t_1, ..., t_M)}(\bx) \defas G_1^{t_1}\cdots G_M^{t_M}(\bx),
\end{align}
Now that we have defined the $(T_1, ..., T_M)$-periodic tensor transformation $G$. If a kernel $k$ is $G_m$-invariant for all $m=1,...,M$, then $k$ is $G$-invariant. 

We define the kernel Fourier series correspondingly. Let $(t_1, ..., t_M)$ be the tensor index, we compute the kernel harmonics from multidimensional DFT,
\begin{align}
    &k_{(t_1, ..., t_M)}(\bx, \bx') \notag \\
    &= \sum_{s_1=0}^{T_1 - 1} \cdots \sum_{s_M=0}^{T_M - 1} \prod_{m=1}^M \bF^{(m)}_{t_m, s_m} k(\bx, G^{(s_1, ..., s_M)}(\bx')), \notag
\end{align}
where $\bF^{(m)} = [\frac{1}{T_m} e^{-i \frac{2\pi t_m s_m}{T_m}}]_{t_m, s_m=0}^{T_m-1}$ is the DFT matrix for the $m$-th transformation. 

%In previous subsections, we have shown the invariance properties for inner product kernels and stationary kernels. Therefore, we can obtain continuous kernel Fourier transforms for them as well. Specifically we will recover the Bochner's theorem for stationary kernels.
%
%\textbf{Recovering Bochner's theorems.} Given a stationary kernel $k(\bx, \bx') = \tau(\bx - \bx')$, we can comptue the kernel Fourier transform. Specifically, we consider $M=d$ transformations that $G_m$ is the periodic translation we proposed applied on $\bx_m$. Taking the limit of $a \to \infty$, the kernel Fourier transformation of $\tilde{k}$ can be written as, 
%\begin{align}
%    \tilde{k}_{t}(\bx, \bx') %&= \int_{\Reals^d} e^{-2\pi i \bs^{\top}\bt} \tilde{k}(\bx, \bx'+\bs) \mathrm{d}\bs \notag \\
%    &= \int_{\Reals^d} e^{-2\pi i \bt^{\top}\bs } \tau (\gamma(\bx - \bx' - \bs)) \mathrm{d}\bs  \notag \\
%    &= \int_{\Reals^d} e^{-2\pi i  \bt^{\top} (\bx - \bx'-\bs)} \tau(\gamma(\bs)) \mathrm{d}\bs  \notag \\
%    &= e^{-2\pi i  \bt^{\top} (\bx - \bx')} \int_{\Reals^d}e^{2\pi i  \bt^{\top} \bs} \tau(\gamma(\bs)) \mathrm{d}\bs \notag \\
%    &=  e^{-2\pi i  \bt^{\top} (\bx - \bx')} \fourierT^{-1}(\tau \circ \gamma)(\bt).
%\end{align}
%Where $\fourierT^{-1}$ is the inverse Fourier transform. Because the kernel sum decomposition, we obtain that,
%\begin{align}
%    \tilde{k}(\bx, \bx') = \int_{\Reals^d} k_\bt(\bx, \bx') \mathrm{d} \bt = \int_{\Reals^d} e^{-2\pi i  \bt^{\top} (\bx - \bx')} \fourierT^{-1}(\tau \circ \gamma)(\bt) \mathrm{d}\bt.
%\end{align}
%This resembles Bochner's theorem except that we consider the extended kernel $\tilde{k}$. \ssy{need to be more careful with the limitation}
%
%\textbf{Inner product kernels.} For inner product kernels, we consider the rotation transformation $G^{\bs}, \bs \in \Sphere^{d-1}$. Let an anchor point be $\be_1 = [1, 0, ..., 0]$, then the transformation $G^{\bs}(\bx) = \bs-\be_1 + \bx$
%
%
%For inner product kernel, we also let $M=d$ and let $G_m$ affect $\bx_m$ only: $G_m^{s_m}(\bx_m) = e^{2\pi i s_m} \bx_m$. Then we can compute the kernel Fourier transform, 
%\begin{align}
%     k_{t}(\bx, \bx') 
%     &= \int_{[0,1]^d} e^{-2\pi i \bs^{\top}\bt} k(\bx, e^{2\pi i \bs} \circ \bx') \mathrm{d}\bs,
%\end{align}
%

%
%\subsection{Inner-product Kernel Decomposition}
%Inner-product kernels are kernels of the form,
%\begin{align}
%    k(\bx, \bx') = \kappa(\bx^{\star}\bx, \bx^{\star}\bx', \bx'^{\star}\bx'),
%\end{align}
%For any matrix $\bR \in \Complex^{d \times d}$, which is unitary $\bR \bR^{*} = \bI$ and $\bR^{T} = \bI$, the mapping $G(\bx) = \bR \bx$ is a $T$-periodic transformation. Because $\bR$ is unitary, the kernel $k$ is $G$-invariant,
%\begin{align}
%    k(G(\bx), G(\bx')) &= \kappa(\bx^{\star} \bR^\star \bR \bx, \bx^{\star} \bR^\star \bR \bx', \bx'^{\star} \bR^\star \bR  \bx') \notag \\
%    &= \kappa(\bx^{\star}\bx, \bx^{\star}\bx', \bx'^{\star}\bx') \notag,
%\end{align}
%Therefore, we can compute the kernel Fourier series,
%\begin{align}
%k_t(\bx, \bx') =  \sum_{s=0}^{T-1} \bF_{t, s} k(\bx, \bR ^s(\bx')).
%\end{align}
%$k_t$ captures the $t$-th harmonic of the kernel $k$ along the sequence by left-multiplications of $\bR$.


\subsection{Kernel Fourier Transform}
We have shown that the Fourier series of length $T$ decomposes the kernel into $T$ orthogonal kernels based on the frequencies. Intuitively, if we let $T \to \infty$, then we obtain a continuous frequency representation of the kernel, which would be akin to a Fourier transform. In this subsection, we present rigorous evidences to connect the kernel Fourier series with kernel Fourier transform. % In particular, we generalize the Fourier transformation from stationary kernels and zonal kernels to any $G$-invariant kernels of some periodic transformation $G$.

Consider the transformation $G^\bs: \xdomain \to \xdomain, \bs \in \bR^M$, where $M\geq 1$ corresponds to the multi-dimensional transformations. $G$ is periodic with period $\bone$: $G^\bzero(\bx)=G^\bone(\bx)=\bx, G^{\bs_1+\bs_2}(\bx)=G^{\bs_1}(G^{\bs_2}(\bx)), \forall \bs_1, \bs_2 \in \Reals^M$. A kernel is $G$-invariant if for any $\bs \in \bR^M$, $k(G^\bs(\bx), G^\bs(\bx')) = k(\bx, \bx')$. Then we define the \emph{kernel Fourier transform} as the following: for $\bt \in \Reals^M$,
\begin{align}
    k_{\bt}(\bx, \bx') = \int_{[0,1]^M} e^{-2\pi i \bs^{\top}\bt} k(\bx, G^\bs(\bx')) \mathrm{d}\bs,
\end{align}
Therefore, $k_\bt(\bx, \bx')$ captures the frequency $\bt$  of the function $\bs \to k(\bx, G^\bs(\bx'))$. Similar to kernel series, the kernel Fourier transform is an alternative representation of $k$, as shown in the following theorem.
\begin{theorem}[Kernel Frequency Representation]\label{thm:kern-ft}
\begin{align}
    k(\bx, \bx') = \int_{\Reals^M} k_\bt(\bx, \bx') \mathrm{d} \bt.
\end{align}
Moreover, $k_\bt$ is a kernel for all $\bt \in \Reals^M$.
\end{theorem}
The proof can be found in Subsection~\ref{app:subsec:proof-kern-ft} in the appendix.


==> kern-tex/spectral-analysis.tex <==
\section{Kernel Spectral Analysis}

==> kern-tex/spectral-decoupled-inference-legacy.tex <==
\section{Spectrally Decomposed Variational Gaussian Processes}
In this section, we explore the implications of the kernel orthogonal decomposition, and propose the \emph{Spectrally Decomposed Variational Gaussian Processes (SDVGP)}, an inference strategy for stochastic variational Gaussian processes. 


\subsection{Decoupled Variational Inference}
Given the kernel decomposition $k = \sum_{t=0}^{T-1} k_t$ \footnote{$t$ can be a multi-index for multi-dimensional transformations.}, the Gaussian Processes $\GP(0, k)$ can be reformulated as,
\begin{align}\label{eq:additive-gp}
    f = \sum_{t=0}^{T-1} f_t, \; f_t \sim \GP(0, k_t), t=0,...,T-1
\end{align}
Given the GP decomposition, SDVGP uses a variational posterior separately for each GP, similarly to \citet{shi2020sparse}. Specifically, for $t=0,...,T-1$, let $\bu_t$ be inducing variables on $\bZ_t$ and $q_t(\bu_t) = \normal(\bmu_t, \bS_t)$ be the variational posterior of $\bu_t$, then the overall variational posterior can be formulated as,
\begin{align} \label{eq:q-k}
    f &= \sum_{t=0}^{T-1} f_t, \\
    q_t(f_t, \bu_t) &= p_t(f_t | \bu_t) q_t(\bu_t), t=0,...,T-1, \notag 
\end{align}
where $p_t$ represents the Gaussian Process $\GP(0, k_t)$. Specifically, if each $q_t$ uses $m$ inducing points, we term the model as a $T\times m$ model. The variational posterior can be optimized by maximizing the Evidence Lower Bound (ELBO),
\begin{align}
    \elbo \defas \expect_{q(f, \bu)} [\log p(\by|f, \bX)] & - \sum_{t=0}^{T-1} \KL{q_t(\bu_t)}{p(\bu_t)}. \notag 
\end{align}

\subsection{Approximation Capacity}\label{subsec:appr-capa}
How well does the decoupled variational inference approximate the true posterior, compared to the standard SVGP? This question boils down to two questions, 
\begin{itemize}
\item \textbf{Kernel Approximation.} How well do decoupled inducing points $\{\bZ_t\}_{t=0}^{T-1}$ approximate the kernel $k$ ?
\item \textbf{Posterior Approximation.} How well does the decoupled variational posterior $\prod_{t=0}^{T-1} q_t(\bu_t)$ approximate the optimial posterior $q^{\star}(\{\bu_t\}_{t=0}^{T-1})$? 
\end{itemize}

\textbf{Kernel Approximation.} Intuitively, how well does the Nystrom approximation using $\bZ$ approximates the kernel, depends on how large is the space spanned by $k(\bx, \bZ)$. For decoupled inducing points, the space is then $\text{span}\{k_t(\bx, \bZ_t)\}_{t=0}^{T-1}$. We let $\bZ_0 =  \cdots \bZ_{T-1} =: \tilde{\bZ}$, since the Fourier series is a bijective linear operation, 
\begin{align}
    \text{span}\{k_t(\bx, \bZ_t)\}_{t=0}^{T-1} = \text{span}\{k(\bx, G^{t}(\tilde{\bZ}))\}_{t=0}^{T-1}, \notag 
\end{align}
Therefore, the decoupled inducing points $\{\bZ_t\}_{t=0}^{T-1}$ approximate the kernel at least as well as the standard inducing points $\{G^t(\tilde{\bZ})\}_{t=0}^{T-1}$. If the transformation $G$ is set so that $\{G^t(\tilde{\bZ})\}_{t=0}^{T-1}$ covers the input domain well, then the decoupled inducing points approximate the kernel accurately.

%The Nystrom approximation error $\expect_{\bx}[k(\bx, \bx) - k(\bx, \bZ) k(\bZ, \bZ)^{-1} k(\bZ, \bx)]$ is a key proxy for evaluating kernel approximations \citep{titsias2009variational, burt2019rates}. 

\textbf{Posterior Approximation.} Given the decoupled inducing points, the optimal posterior covariance is $\bS^{\star} \in \Reals^{TM \times TM}$, while we induce a block diagonal structure in SDVGP. However, we can show that $\bS^{\star}$ is approximately block diagonal indeed if the input distribution is invariant to $G$.

\begin{lemma}\label{lem:decoupled} If the data distribution is invariant to $G$, i.e.,
\begin{align}
    \forall \bx, p(G(\bx)) = p(\bx),
\end{align}
Then $\bS^{\star}$ becomes block diagonal when the training size $N \to \infty$.
\end{lemma}
%\begin{remark} Because the transformation is a rigid rotation around the origin, the assumption is satisfied by many data distributions, such as the uniform distribution and the isotropic normal distribution.
%\end{remark}
%\begin{remark} This lemma demonstrates that the whitening preprocess (subtracting by the mean, dividing by the standard deviation) is necessary.
%\end{remark}
The proof can be found in Subsection~\ref{app:prof:lemma-dvi} in the appendix. This lemma highlights that, if the density of the data distribution is approximately invariant to the transformation $G$, then the decoupled variational posterior induces little error compared to the optimal posterior.

Summing up the analyses in kernel approximation and posterior approximation, we conclude that the SDVGP approximates the true GP posterior accurately when \emph{the trajectories under the transformation $G$ cover the input domain well}. We illustrate this gist by a \textit{flip-mnist} dataset, where each digit in the MNIST dataset is randomly flipped up-and-down or left-and-right. For a RBF kernel, we consider two variations of SDVGP in terms of the transformation. 1) Negation. We split input dimensions into two groups and negate them separately, resulting in a $4\times 100$ model. 2) Flipping the image up-and-down or left-and-right, resulting in a $4\times 100 $ model. We compare them with the standard SVGP using $100, 400$ inducing points, shown in Figure~\ref{fig:flipmnist}.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/flipmnist_M100_reordered_two.pdf}
\caption{Flip-mnist.  From left to right, we plot how \textit{train loss}, \textit{test acc} and \textit{test lld} evolve with training. We observe SDVGP using \textit{FLIP: $4 \times 100$} performs on par with standard SVGP using \textit{$400$} inducing points while SDVGP using \textit{NEG: $4 \times 100$} performs substantially worse. This experiment highlights the importance of matching the transformation $G$ with the data distribution. \label{fig:flipmnist}}
\end{figure} 

\subsection{Computational Costs}

\textbf{Computational Costs.} The computational costs boil down to the cost of 
computing $k_t(\bZ_t, \bZ_t)$ and the cost of decoupled variational inference. Let $T\times m$ represents using $m$ inducing points for each $t=0, ..., T-1$, and assume the mini-batch size $n = \bigO(m)$. The computational cost of decoupled variational inference is then $\bigO(T m^3)$; To compute $k_t(\bZ_t, \bZ_t)$, we need the kernel values $k(\bZ_t, G^s(\bZ_t))$ for $s=0,...,T-1$. If $c_G$ represents the cost of applying $G$, then computing $\bK_{\bu, \bu}$ requires $\bigO(Tm \times T c_G + Tm^2 \times T)$ operations. Therefore, the overall computational cost is
\begin{align}
    \bigO(T m^3  + T^2 m^2 + T^2 m c_G),
\end{align}
When $T \ll m$, the cost scales approximately linearly with $T$. Furthermore, the proposed SDVGP supports parallel computations straightforwardly: we can locate all computations of $k_t$ on the $t$-th device and enjoy the parallelism.

\textbf{Memory Costs.}  The memory cost overhead stems from computing the kernel matrix $\bK_{\bu\bu}$. For computing $\bK_{\bu\bu}$, we need the kernel values $k(\bZ_t, G^s(\bZ_t))$ for $s=0,...,T-1$, which implies the memory cost $\bigO(T \times m^2 \times T)$. Since the memory cost of decoupled variational inference is $\bigO(T \times m^2)$, the overall memory cost is,
\begin{align}
    \bigO(T^2m^2),
\end{align}

\textbf{Storage Costs.} Storing a $T\times m$ model needs to keep $T$ variational posteriors, requiring $\bigO(Tm^2 + Tmd)$ storage.

%\subsection{The Transformation $G$}
%Our kernel decomposition framework provides wide modelling choices for choosing the transformation $G$. For example, one can choose which axis to rotate round; one can choose the period $T$; one can combine multiple $G$s to form a multi-dimensional transformation. Given the analyses of the approximation capacity in Subsection~\ref{subsec:appr-capa}, the SDVGP approximates the true posterior well if 1) Nystrom approximation using the inducing points $\{G^t(\bZ)\}_{t=0}^{T-1}$ approximates the kernel well; 2) the data distribution is approximately invariant to $G$.
%
%As shown in Subsection~\ref{subsec:example}, both stationary kernels and inner-product kernels are invariant to the negation $G(\bx)=-\bx$. We consider the multi-dimensional composition of negations. For example, if $\bx=[\bx_1, \bx_2]^{\top} \in \Reals^2$, the two-dimensional transformations are $G^{(0,0)}(\bx)=[\bx_1, \bx_2]^{\top}, G^{(0,1)}(\bx)=[\bx_1, -\bx_2]^{\top}, G^{(1,0)}(\bx)=[-\bx_1, \bx_2]^{\top}, G^{(1,1)}(\bx)=[-\bx_1, -\bx_2]^{\top}$. For higher dimensional inputs, we can split the input dimension into $J$ groups and conduct group-wise negations, then we decompose the kernel into $T = 2^J$ kernels.
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.5\textwidth]{figures/pca1.pdf}
%\caption{Comparing transformations along axes (left) and along principled directions (right). The shaded area represents the data distribution. We observe that $G^{1,0}(\bx), G^{0,1}(\bx)$ are out of the data distribution when transforming along axes. In comparison, when transforming along principled directions, $G^{0,0}(\bx), G^{1,0}(\bx), G^{0,1}(\bx), G^{1,1}(\bx)$ are all in-distribution and has the same density.\label{fig:pca}}
%\end{figure}
%
%However, if the data distribution is not isotropic, $G^{(0,1)}(\bx)=[\bx_1, -\bx_2]^{\top}$ might be out-of-distribution. To make the $\{G^t(\bZ)\}_{t=0}^{T-1}$ spread over the input space, we can conduct negations along the principle component  analysis (PCA) directions. Moreover, if the input distribution is a zero-mean Gaussian,  not only negating along principle direction makes $G(\bZ)$ in-distribution, the input distribution is also invariant to $G$. This property is visualized in Figure~\ref{fig:pca}.

\subsection{Resolving Hermitian Kernels}\label{subsec:resolve-hermitian}
Our orthogonal kernel decomposition arises from the discrete Fourier transform, thus $k_t$ is Hermitian but not necessarily real-valued. This elicits the difficulty for $k_t$ to be used in Gaussian processes as a GP is commonly defined as a real process \citep{rasmussen2006gaussian}. So when is $k_t$ not real-valued and how can we resolve this issue ? 

For a single dimensional transformation, the DFT matrix $\bF = [\frac{1}{T} e^{-i\frac{2\pi t s}{T} } ]_{t,s=0}^{T-1}$. Then the  DFT introduces imaginary values whenever $T > 2$. For $M$-dimensional transformations where $t = (t_1, ..., t_M)$ is a multi-index, subsection~\ref{subsec:multi-dim} shows that the DFT matrix is the tensor product of all single-dimensional DFT matrices. Thus the DFT introduces imaginary values whenever $T_m > 2$ for some $1\leq m\leq M$. Therefore, rotations by $90^{\text{o}}$ in Figure~\ref{fig:rbf-rotate-gp} does introduce imaginary values because its period is $4$, but flipping left-right and up-down in Figure~\ref{fig:flipmnist} does not because it involves only period $2$ transformations.

Fortunately we can resolve Hermitian kernels to be all real-valued. Consider a single dimensional transformation with period $T$, we sum up $k_t$ and $k_{T-t}$ together,
\begin{align}
    (k_t + k_{T-t})(\bx, \bx') = \sum_{s=0}^{T-1} \left(\bF_{t, s}+\bF_{T-t, s} \right) k(\bx, G^s(\bx')), \notag
\end{align}
Because $\bF_{t, s}+\bF_{T-t, s} = \frac{2}{T} \cos(\frac{2\pi t s}{T})$, $k_t + k_{T-t}$ is a real-valued kernel. By pairing up all Hermitian kernels, we obtain a real-valued orthogonal kernel decomposition,
\begin{align}
    k(\bx, \bx') = \sum_{t=0}^{\lfloor T/2 \rfloor+1} \left(k_t + k_{T-t}\right)(\bx, \bx') .
\end{align}
Similarly, for $M$-dimensional transformations with periods $(T_1, ..., T_M)$, we can obtain a real-valued decomposition with $(\lfloor T_1/2 \rfloor+1) \times \cdots \times (\lfloor T_M/2 \rfloor+1)$ kernels.
 

